Exact Gaussian--Hermite closure of the mapping quantum--classical Liouville equation

In the Meyer--Miller--Stock--Thoss mapping representation, the Liouville operator of the quantum--classical Liouville equation contains an excess coupling term in addition to the Poisson bracket. Neglecting this term yields the Poisson bracket mapping equation (PBME). We expand the mapping dependence of the density in Hermite functions about the Gaussian factor common to all physical mapping densities. In this basis, the excess coupling term acts purely as a raising operator and exactly cancels the raising contribution generated by the back--reaction force. Consequently, the exact dynamics does not generate higher Hermite orders and closes on a finite, sparse system of equations for the coefficient fields. Within the physical sector, these equations reduce to the subsystem quantum--classical Liouville equation. In contrast, the PBME retains the raising contribution of the force, modifying the back reaction within the physical sector while continuously generating higher Hermite orders. For Tully's dual avoided crossing model, direct propagation of the coefficient equations confirms this finite closure and agrees with independent solutions of the subsystem equation. Comparison with converged full quantum dynamics further shows that, across all regimes examined, the PBME is less accurate than the quantum--classical description for populations, coherences, and momentum distributions.

==> main_references.tex <==
\makeatletter
\newlabel{M-eq:D4}{{19}{5}{}{}{}}
\newlabel{M-eq:Hm}{{3}{2}{}{}{}}
\newlabel{M-eq:PBcoeff}{{16}{4}{}{}{}}
\newlabel{M-eq:RG}{{14}{4}{}{}{}}
\newlabel{M-eq:T}{{12}{3}{}{}{}}
\newlabel{M-eq:coeff}{{13}{4}{}{}{}}
\newlabel{M-eq:eps}{{15}{4}{}{}{}}
\newlabel{M-eq:force-split}{{11}{3}{}{}{}}
\newlabel{M-eq:inframe}{{17}{4}{}{}{}}
\newlabel{M-eq:mqcle-excess}{{7}{3}{}{}{}}
\newlabel{M-eq:mqcle-full}{{5}{3}{}{}{}}
\newlabel{M-eq:qcle}{{2}{2}{}{}{}}
\newlabel{M-eq:qcle-op}{{1}{2}{}{}{}}
\newlabel{M-eq:quartic}{{18}{5}{}{}{}}
\newlabel{M-eq:raise}{{9}{3}{}{}{}}
\newlabel{M-eq:rhophys}{{4}{2}{}{}{}}
\newlabel{M-fig:ladder}{{1}{5}{}{}{}}
\newlabel{M-fig:numerics}{{2}{8}{}{}{}}
\newlabel{M-fig:phasespace}{{5}{13}{}{}{}}
\newlabel{M-sec:closure-results}{{IV\,A}{6}{}{}{}}
\newlabel{M-sec:physical}{{II\,D}{4}{}{}{}}
\newlabel{M-sec:raising}{{II\,C}{3}{}{}{}}
\newlabel{M-sec:theory}{{II}{2}{}{}{}}
\newlabel{M-tab:params}{{I}{7}{}{}{}}
\makeatother

